State of the Art Report: Verified Computation

This report describes the state of the art in verifiable computation. The problem being solved is the following: The Verifiable Computation Problem (Verifiable Computing Problem) Suppose we have two computing agents. The first agent is the verifier, and the second agent is the prover. The verifier wants the prover to perform a computation. The verifier sends a description of the computation to the prover. Once the prover has completed the task, the prover returns the output to the verifier. The output will contain proof. The verifier can use this proof to check if the prover computed the output correctly. The check is not required to verify the algorithm used in the computation. Instead, it is a check that the prover computed the output using the computation specified by the verifier. The effort required for the check should be much less than that required to perform the computation. This state-of-the-art report surveys 128 papers from the literature comprising more than 4,000 pages. Other papers and books were surveyed but were omitted. The papers surveyed were overwhelmingly mathematical. We have summarised the major concepts that form the foundations for verifiable computation. The report contains two main sections. The first, larger section covers the theoretical foundations for probabilistically checkable and zero-knowledge proofs. The second section contains a description of the current practice in verifiable computation. Two further reports will cover (i) military applications of verifiable computation and (ii) a collection of technical demonstrators. The first of these is intended to be read by those who want to know what applications are enabled by the current state of the art in verifiable computation. The second is for those who want to see practical tools and conduct experiments themselves.

==> Yao.tex <==
Yao's garbled circuits protocol is one of the most prominent early attempts to solve the problem of outsourced computation~\cite{Goldreich&87}. The general idea behind the protocol is to transform functions into Boolean circuits (circuits consisting of AND, OR and NOT gates) with masked inputs. Furthermore, the communicating parties use an oblivious transfer protocol to ensure that the inputs transferred to these Boolean circuits remain hidden. 

The oblivious transfer protocol ensures that, whilst one client receives an input, the other does not know which input was provided. This could be carried out as follows. The first client $\clz cl_1$ has several inputs (let us consider two): $\clz i_0,i_1$. The first client provides an input to the second client $\clz cl_2$, where $\clz cl_2$ wants to hide which input was received from $\clz cl_1$. To this end, $\clz cl_1$ generates an RSA key pair and two random values $\clz v_0,v_1$ and sends them to $\clz cl_2$, including the modulus $\clz N$ and public exponent $\clz e$. Once data from $\clz cl_1$ is received, $\clz cl_2$ picks a binary value $\clz b$, selects $\clz v_b$, and generates a random value $\clz r$. This masks the selection by computing $\clz x = (v_b + r^e) \mod N$ and sends $\clz x$ to $\clz cl_1$. Upon receiving this, $\clz cl_1$ then combines $\clz x$ with generated random values $\clz v_0,v_1$ as $\clz r_0=(x-v_0)^d \mod N$ and $\clz r_1=(x-v_1)^d \mod N$ where $\clz d$ is a private exponent generated by $\clz cl_1$. One of the values will then be equal to $\clz r$, but which one is unknown to $\clz cl_1$ since the value of $\clz b$ is hidden. The two inputs that $\clz cl_1$ is sending are then combined with the possible keys as $\clz i_0'=i_0+r_0$ and $\clz i_1'=i_1+r_1$ and are sent to $\clz cl_2$. Now, since $\clz cl_2$ knows the value $\clz r$, it can compute $\clz i_b = i_b' - r$. This obtains the selected input without the ability to compute the input for $\clz r(1-b)$ since $\clz d$ is only known to $\clz cl_1$. This protocol is used within the wider Yao's garbled circuit protocol as follows:

Consider two clients trying to compute a function $\clz f$ while ensuring that the inputs to the function remain secret. This is accomplished by converting $\clz f$ to an equivalent Boolean circuit $\clz C$, such that 
% $\clz \forall(x,y) \xrightarrow{} f(x,y) = C(x,y)$
$\clz \forall x, y.\ f(x,y) = C(x,y)$.

To do this, the first client $\clz cl_1$ replaces the Boolean values within the circuit with pseudo-random values and saves the mapping of the actual Boolean values to the pseudo-random values for later use. This mapping is kept secret by $\clz cl_1$, meaning that $\clz cl_1$ must possess a mechanism to store the mapping during the lifetime of the computation securely. The garbling is done for every input and output of the circuit's internal gates. In contrast, the final output of the circuit is not garbled (i.e., the result is presented without being misinterpreted). This garbled circuit $\clz g(C)$ and the garbled input $\clz g(cl_{1,i})$ are then sent to the client $\clz cl_2$ (for simplicity, we consider both computing entities as clients as they are within the same level of hierarchy). The client $\clz cl_2$ receives the circuit and the inputs from $\clz cl_1$ without knowing what inputs will be present at the input of the gates within the circuit. To obtain the necessary information, the client $\clz cl_2$ initiates a series of oblivious transfers with $\clz cl_1$, where the oblivious transfer protocol keeps $\clz cl_1$ from finding out what value was selected by $\clz cl_2$ and $\clz cl_2$ from finding out the other possible values that could have been selected~\cite{Naor&01}. $\clz cl_2$ obtains the necessary input $\clz g(cl_{2,i})$, while $\clz cl_1$ learns nothing about the input of $\clz cl_2$. With the complete input and circuit information, $\clz cl_2$ can compute the output of the garbled circuit. This is done by inserting the garbled inputs into specific gates and using their garbled outputs as input for the next gate within the circuit. $\clz cl_2$ processes all the circuit gates and retrieves the output of the final gate, which is not warped. This is then provided to $\clz cl_1$ as a result of the computation. A simple garbled gate is shown in Figure~\ref{fig:garbled}. The inputs and outputs of the original and the garbled gate follow a truth table as shown in Table~\ref{tab:garbled}.

\begin{figure}
\label{tab:garbled}
\caption{Table of computation of garbled values for an OR gate using the hash function $\clz H$}
\centering
\begin{tabular}{|c|c|c|} 
  \hline
  $\clz i_0$& $\clz i_1$ & $\clz o_0$ \\ 
  \hline \hline
  0 & 0 & 0 \\ 
  \hline
  0 & 1 & 1 \\ 
  \hline
  1 & 0 & 1 \\
  \hline
  1 & 1 & 1\\
  \hline
\end{tabular}
$\clz \xrightarrow{}$
\begin{tabular}{|c|c|c|c|} 
  \hline
  $\clz i_0$& $\clz i_1$ & $\clz o_0$ & Garbled \\ 
  \hline \hline
  $\clz k_0^0$ & $\clz k_1^0$ & $\clz k_2^0$ & $\clz H(k_0^0 || k_1^0 ||g_1) \oplus k_2^0$ \\ 
  \hline
  $\clz k_0^0$ & $\clz k_1^1$ & $\clz k_2^1$ & $\clz H(k_0^0 || k_1^1 ||g_1) \oplus k_2^1$ \\ 
  \hline
  $\clz k_0^1$ & $\clz k_1^0$ & $\clz k_2^1$ & $\clz H(k_0^1 || k_1^0 ||g_1) \oplus k_2^1$ \\
  \hline
  $\clz k_0^1$ & $\clz k_1^1$ & $\clz k_2^1$ & $\clz H(k_0^1 || k_1^2 ||g_1) \oplus k_2^1$\\
  \hline
\end{tabular}
\end{figure}

Note the protocol's security aspects. One of the main challenges in using Yao's garbled circuit protocol is that its design works in an environment with \emph{semi-honest} adversaries, which practically excludes it for use within high-stake outsourced computation. This led to developments in ways to modify the protocol to function within the environment with \emph{malicious} adversaries. The first thing to ensure is that the client constructing the garbled circuit does it correctly. Several approaches were proposed, such as zero-knowledge proofs~\cite{Goldreich&94} and cut-and-choose approaches~\cite{Kolesnikov&17}. Several of these approaches are discussed in detail in this report. Another aspect is improving the security of the oblivious transfer protocol. One of the potential security issues is that $\clz cl_2$ could potentially generate private and public keys in such a way that it could obtain the non-garbled values sent by $\clz cl_1$. Several solutions have been proposed to secure against such issues~\cite{Beaver&98}, while oblivious transfer is still an active research topic. Finally, a security issue could be noted where $\clz cl_1$ can send corrupted values to $\clz cl_2$. A protection for this was proposed where the input bits are extended with more input bits and a security parameter~\cite{Lindell&07} and then replaced the input bits by the XOR of the security parameter input bits. 

Yao's garbled circuit protocol is one of the early steps towards the techniques described within this report to reach secure, verifiable, outsourced computation in potentially hostile environments. The research into fast multiparty computation creates new schemes focusing on computational practicality. It has also been shown that the protocol could be made secure in a scenario with malicious adversaries using zero-knowledge proofs (described in~\ref{sec:pokzk}).

\begin{figure}
  \centering
  \begin{circuitikz} \draw
    (0,1) node[or port] (myor1) {}
    (myor1.in 1) node [anchor=east] {$\clz i_0$}
    (myor1.in 2) node [anchor=east] {$\clz i_1$}
    (myor1.out) node [anchor=west] {~$\clz o_0$}
    (5,1) node[or port] (myor2) {}
    (myor2.in 1) node [anchor=east] {$\clz k_0^0,k_1^0$}
    (myor2.in 2) node [anchor=east] {$\clz k_0^1,k_1^1$}
    (myor2.out) node [anchor=west] {~$\clz k_0^2,k_1^2$}
    [-latex](1,1) -- (2,1);
  \end{circuitikz}
  \caption{Original gate transformed to garbled gate\\\null}
  \label{fig:garbled}
\end{figure}


